How to think step-by-step: A mechanistic understanding of chain-of-thought reasoning

Despite superior reasoning prowess demonstrated by Large Language Models (LLMs) with Chain-of-Thought (CoT) prompting, a lack of understanding prevails around the internal mechanisms of the models that facilitate CoT generation. This work investigates the neural sub-structures within LLMs that manifest CoT reasoning from a mechanistic point of view. From an analysis of Llama-2 7B applied to multistep reasoning over fictional ontologies, we demonstrate that LLMs deploy multiple parallel pathways of answer generation for step-by-step reasoning. These parallel pathways provide sequential answers from the input question context as well as the generated CoT. We observe a functional rift in the middle layers of the LLM. Token representations in the initial half remain strongly biased towards the pretraining prior, with the in-context prior taking over in the later half. This internal phase shift manifests in different functional components: attention heads that write the answer token appear in the later half, attention heads that move information along ontological relationships appear in the initial half, and so on. To the best of our knowledge, this is the first attempt towards mechanistic investigation of CoT reasoning in LLMs.

==> tokenized.tex <==
{\tt
<s>\_0
<s>\_1
<s>\_2
<s>\_3
<s>\_4
<s>\_5
\#\#\#\_6
Input\_7
:\_8
<0x0A>\_9
G\_10
or\_11
pus\_12
is\_13
tw\_14
imp\_15
us\_16
.\_17
Alex\_18
is\_19
rom\_20
pus\_21
.\_22
Rom\_23
pus\_24
is\_25
g\_26
or\_27
pus\_28
.\_29
Gor\_30
pus\_31
is\_32
small\_33
.\_34
Rom\_35
pus\_36
is\_37
mean\_38
.\_39
True\_40
or\_41
false\_42
:\_43
Alex\_44
is\_45
small\_46
.\_47
Let\_48
us\_49
think\_50
step\_51
by\_52
step\_53
.\_54
<0x0A>\_55
\#\#\_56
\#\_57
Response\_58
:\_59
<0x0A>\_60
Alex\_61
is\_62
rom\_63
pus\_64
.\_65
Rom\_66
pus\_67
is\_68
g\_69
or\_70
pus\_71
.\_72
Alex\_73
is\_74
g\_75
or\_76
pus\_77
.\_78
Gor\_79
pus\_80
is\_81
small\_82
.\_83
Alex\_84
is\_85
small\_86
.\_87
True\_88
<0x0A>\_89
<0x0A>\_90
\#\#\_91
\#\_92
Input\_93
:\_94
<0x0A>\_95
G\_96
orp\_97
uses\_98
are\_99
disc\_100
ord\_101
ant\_102
.\_103
Max\_104
is\_105
zum\_106
pus\_107
.\_108
Z\_109
ump\_110
us\_111
is\_112
sh\_113
amp\_114
or\_115
.\_116
Z\_117
ump\_118
us\_119
is\_120
g\_121
or\_122
pus\_123
.\_124
Gor\_125
pus\_126
is\_127
earth\_128
y\_129
.\_130
True\_131
or\_132
false\_133
:\_134
Max\_135
is\_136
small\_137
.\_138
Let\_139
us\_140
think\_141
step\_142
by\_143
step\_144
.\_145
\_146
<0x0A>\_147
\#\#\_148
\#\_149
Response\_150
:\_151
<0x0A>\_152
Max\_153
is\_154
zum\_155
pus\_156
.\_157
Z\_158
ump\_159
us\_160
is\_161
g\_162
or\_163
pus\_164
.\_165
Max\_166
is\_167
g\_168
or\_169
pus\_170
.\_171
Gor\_172
p\_173
uses\_174
are\_175
disc\_176
ord\_177
ant\_178
.\_179
Max\_180
is\_181
disc\_182
ord\_183
ant\_184
.\_185
False\_186
<0x0A>\_187
<0x0A>\_188
\#\#\_189
\#\_190
Input\_191
:\_192
<0x0A>\_193
B\_194
or\_195
pin\_196
are\_197
w\_198
ump\_199
us\_200
.\_201
W\_202
ump\_203
uses\_204
are\_205
angry\_206
.\_207
W\_208
ump\_209
us\_210
is\_211
j\_212
empor\_213
.\_214
S\_215
ally\_216
is\_217
le\_218
mp\_219
us\_220
.\_221
L\_222
emp\_223
us\_224
is\_225
w\_226
ump\_227
us\_228
.\_229
True\_230
or\_231
false\_232
:\_233
S\_234
ally\_235
is\_236
fl\_237
oral\_238
.\_239
Let\_240
us\_241
think\_242
step\_243
by\_244
step\_245
.\_246
\_247
<0x0A>\_248
\#\#\_249
\#\_250
Response\_251
:\_252
<0x0A>\_253
S\_254
ally\_255
is\_256
le\_257
mp\_258
us\_259
.\_260
L\_261
emp\_262
us\_263
is\_264
w\_265
ump\_266
us\_267
.\_268
S\_269
ally\_270
is\_271
w\_272
ump\_273
us\_274
.\_275
W\_276
ump\_277
uses\_278
are\_279
angry\_280
.\_281
S\_282
ally\_283
is\_284
angry\_285
.\_286
False\_287
<0x0A>\_288
<0x0A>\_289
\#\#\_290
\#\_291
Input\_292
:\_293
<0x0A>\_294
G\_295
or\_296
pus\_297
is\_298
jel\_299
git\_300
.\_301
Y\_302
ump\_303
uses\_304
are\_305
loud\_306
.\_307
Gor\_308
pus\_309
is\_310
y\_311
ump\_312
us\_313
.\_314
Y\_315
ump\_316
us\_317
is\_318
orange\_319
.\_320
R\_321
ex\_322
is\_323
g\_324
or\_325
pus\_326
.\_327
True\_328
or\_329
false\_330
:\_331
R\_332
ex\_333
is\_334
loud\_335
.\_336
Let\_337
us\_338
think\_339
step\_340
by\_341
step\_342
.\_343
<0x0A>\_344
\#\#\_345
\#\_346
Response\_347
:\_348
<0x0A>\_349
R\_350
ex\_351
is\_352
g\_353
or\_354
pus\_355
.\_356
Gor\_357
pus\_358
is\_359
y\_360
ump\_361
us\_362
.\_363
R\_364
ex\_365
is\_366
y\_367
ump\_368
us\_369
.\_370
Y\_371
ump\_372
uses\_373
are\_374
loud\_375
.\_376
R\_377
ex\_378
is\_379
loud\_380
.\_381
True\_382
<0x0A>\_383
<0x0A>\_384
\#\#\_385
\#\_386
Input\_387
:\_388
<0x0A>\_389
L\_390
emp\_391
us\_392
is\_393
t\_394
ump\_395
us\_396
.\_397
Max\_398
is\_399
le\_400
mp\_401
us\_402
.\_403
T\_404
ump\_405
us\_406
is\_407
f\_408
ru\_409
ity\_410
.\_411
T\_412
ump\_413
us\_414
is\_415
bright\_416
.\_417
L\_418
emp\_419
us\_420
is\_421
drop\_422
ant\_423
.\_424
True\_425
or\_426
false\_427
:\_428
Max\_429
is\_430
bright\_431
.\_432
Let\_433
us\_434
think\_435
step\_436
by\_437
step\_438
.\_439
<0x0A>\_440
\#\#\_441
\#\_442
Response\_443
:\_444
<0x0A>\_445
Max\_446
is\_447
le\_448
mp\_449
us\_450
.\_451
L\_452
emp\_453
us\_454
is\_455
t\_456
ump\_457
us\_458
.\_459
Max\_460
is\_461
t\_462
ump\_463
us\_464
.\_465
T\_466
ump\_467
us\_468
is\_469
bright\_470
.\_471
Max\_472
is\_473
bright\_474
.\_475
True\_476
<0x0A>\_477
<0x0A>\_478
\#\#\_479
\#\_480
Input\_481
:\_482
<0x0A>\_483
S\_484
ter\_485
p\_486
uses\_487
are\_488
d\_489
ull\_490
.\_491
Imp\_492
us\_493
is\_494
medium\_495
.\_496
Imp\_497
uses\_498
are\_499
ster\_500
p\_501
uses\_502
.\_503
W\_504
ren\_505
is\_506
imp\_507
us\_508
.\_509
Ster\_510
pus\_511
is\_512
da\_513
ump\_514
in\_515
.\_516
True\_517
or\_518
false\_519
:\_520
W\_521
ren\_522
is\_523
mel\_524
od\_525
ic\_526
.\_527
Let\_528
us\_529
think\_530
step\_531
by\_532
step\_533
.\_534
<0x0A>\_535
\#\#\_536
\#\_537
Response\_538
:\_539
<0x0A>\_540
W\_541
ren\_542
is\_543
imp\_544
us\_545
.\_546
Imp\_547
uses\_548
are\_549
ster\_550
p\_551
uses\_552
.\_553
W\_554
ren\_555
is\_556
ster\_557
pus\_558
.\_559
Ster\_560
p\_561
uses\_562
are\_563
d\_564
ull\_565
.\_566
W\_567
ren\_568
is\_569
d\_570
ull\_571
.\_572
False\_573
<0x0A>\_574
<0x0A>\_575
\#\#\_576
\#\_577
Input\_578
:\_579
<0x0A>\_580
J\_581
om\_582
pus\_583
is\_584
wooden\_585
.\_586
Imp\_587
us\_588
is\_589
j\_590
om\_591
pus\_592
.\_593
St\_594
ella\_595
is\_596
imp\_597
us\_598
.\_599
True\_600
or\_601
false\_602
:\_603
St\_604
ella\_605
is\_606
wooden\_607
.\_608
Let\_609
us\_610
think\_611
step\_612
by\_613
step\_614
.\_615
<0x0A>\_616
\#\#\_617
\#\_618
Response\_619
:\_620
<0x0A>\_621
St\_622
ella\_623
is\_624
}
